CONTINUUM: Detecting APT Attacks through Spatial-Temporal Graph Neural Networks

Advanced Persistent Threats (APTs) represent a significant challenge in cybersecurity due to their sophisticated and stealthy nature. Traditional Intrusion Detection Systems (IDS) often fall short in detecting these multi-stage attacks. Recently, Graph Neural Networks (GNNs) have been employed to enhance IDS capabilities by analyzing the complex relationships within networked data. However, existing GNN-based solutions are hampered by high false positive rates and substantial resource consumption. In this paper, we present a novel IDS designed to detect APTs using a Spatio-Temporal Graph Neural Network Autoencoder. Our approach leverages spatial information to understand the interactions between entities within a graph and temporal information to capture the evolution of the graph over time. This dual perspective is crucial for identifying the sequential stages of APTs. Furthermore, to address privacy and scalability concerns, we deploy our architecture in a federated learning environment. This setup ensures that local data remains on-premise while encrypted model-weights are shared and aggregated using homomorphic encryption, maintaining data privacy and security. Our evaluation shows that this system effectively detects APTs with lower false positive rates and optimized resource usage compared to existing methods, highlighting the potential of spatio-temporal analysis and federated learning in enhancing cybersecurity defenses.

==> comments.tex <==
%\setcopyright{acmlicensed}
%\copyrightyear{2024}
%\acmYear{2024}
%\acmDOI{XXXXXXX.XXXXXXX}

%% These commands are for a PROCEEDINGS abstract or paper.
%\acmConference[Conference acronym 'XX]{Make sure to enter the correct conference title}{June 03--05,2018}{Woodstock, NY}
%
%  Uncomment \acmBooktitle if th title of the proceedings is different
%  from ``Proceedings of ...''!
%
%\acmBooktitle{Woodstock '18: ACM Symposium on Neural Gaze Detection,
%  June 03--05, 2018, Woodstock, NY} 
%\acmISBN{978-1-4503-XXXX-X/18/06}

%% Submission ID.
%% Use this when submitting an article to a sponsored event. You'll
%% receive a unique submission ID from the organizers
%% of the event, and this ID should be used as the parameter to this command.
%%\acmSubmissionID{123-A56-BU3}


%%
%% The majority of ACM publications use numbered citations and
%% references.  The command \citestyle{authoryear} switches to the
%% "author year" style.
%%
%% If you are preparing content for an event
%% sponsored by ACM SIGGRAPH, you must use the "author year" style of
%% citations and references.
%% Uncommenting
%% the next command will enable that style.
%%\citestyle{acmauthoryear}


%%

%%
%% end of the preamble, start of the body of the document source.

%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
%\begin{CCSXML}
%<ccs2012>
%   <concept>
       %<concept_id>10010520.10010521.10010542.10010294</%concept_id>
  %     <concept_desc>Computer systems %organization~Neural networks</concept_desc>
 %      <concept_significance>500</concept_significance>
 %      </concept>
 %  <concept>
       %<concept_id>10002978.10002997.10002999</concept_i%d>
 %      <concept_desc>Security and privacy~Intrusion %detection systems</concept_desc>
     %  <concept_significance>500</concept_significance>
     %  </concept>
 %  <concept>
       %<concept_id>10002951.10002952.10002971.10003451.1%0002976</concept_id>
       %<concept_desc>Information systems~Data %encryption</concept_desc>
%       <concept_significance>500</concept_significance>
%       </concept>
% </ccs2012>
%\end{CCSXML}

%\ccsdesc[500]{Security and privacy~Intrusion detection systems}
%\ccsdesc[500]{Information systems~Data encryption}
%\ccsdesc[500]{Computer systems organization~Neural networks}

%% the author to define a more concise list
%% of authors' names for this purpose.
%\renewcommand{\shortauthors}{Mansour Bahar and Ferrahi, et al.}

%% The following are not a requirement, delete if not using
%\received{20 February 2024}  %% inital submission date
%\received[revised]{12 March 2024} %% interim new draft
%\received[accepted]{5 June 2024}  %% publication version
